Rigidity of $\mathbf{\textit{U}}$-Gibbs measures near conservative Anosov diffeomorphisms on $\mathbb{T}^3$

We show that within a $C^1$-neighbourhood $\mathcal{U}$ of the set of volume preserving Anosov diffeomorphisms on the three-torus $\mathbb{T}^3$ which are strongly partially hyperbolic with expanding center, any $f\in\mathcal{U}\cap\operatorname{Diff}^2(\mathbb{T}^3)$ satisfies the dichotomy: either the strong stable and unstable bundles $E^s$ and $E^u$ of $f$ are jointly integrable, or any fully supported $u$-Gibbs measure of $f$ is SRB.

==> Sec9_attractors.tex <==
For this section we will assume that $f:M^3 \to M^3$ is a $C^2$-diffeomorphism and  $\Lambda$ is a transitive hyperbolic attractor such that
\begin{enumerate}
\item $T_{\Lambda} M = E^s \oplus E^c \oplus E^u$, where $E^c$ expands uniformly;
\item the stable holonomy $H^s$ is $C^1$, that is, for any $p\in \Lambda $ and  $q\in \cW^s(p)\cap \Lambda$, there is a well defined stable holonomy map $H^s_{p,q}:W^{cu}_{loc}(p) \to  \cW^{cu}_{loc}(q)$ and this map is $C^1$. 
\end{enumerate}



We define in the angle function $\alpha^s(x,y)$ in same way as in  Definition \ref{def_angle-function},  where for attractors we have  $x\in \Lambda$ and $y\in \cW^s(x) \cap \Lambda$.  Given an invariant measure $\mu$, we define in the same way as in Definition \ref{def bad set} the bad set $\mathbf{B} = \mathbf{B}_{\mu}$.  The proof of Theorem \ref{mainthm.technique intro} also works for hyperbolic attractors, in particular, the same proof gives the following statement. 

\begin{theorem}
\label{thm. mainthmforattractors}
Let $f: M^3 \to M^3$ be a $C^2$-diffeomorphism and let $\Lambda$ be a hyperbolic attractor as above.  Let $\mu$  be a $u$-Gibbs measure. If $\mu(\mathbf{B}) = 0$ then $\mu$ is SRB.
\end{theorem}

Theorem \ref{thm. mainthmforattractors} implies the version of Theorem \ref{mainthm.fullsupport} for attractors. 

\begin{theorem}
\label{thm.fullsupportmainthmattractors}
Let $f:M^3 \to M^3$ be a $C^2$ diffeomorphism and let $\Lambda$ be a hyperbolic attractor as above. Then, either
\begin{enumerate}
\item $E^s$ and $E^u$ are jointly integrable, or
\item any fully supported, ergodic $u$-Gibbs measure is SRB.  
\end{enumerate}
\end{theorem}

\subsection{The usu-accessibility property and minimality of the strong unstable lamination}

We say that $\Lambda$ has the  \emph{usu-accessibility} property if any two points $x,y\in \Lambda$ can be connected by a a path with at most three legs in which two are contained in unstable manifolds and one in a stable manifold.   The goal of this subsection is to prove the following theorem. 

\begin{theorem}
\label{thm.attractorusu}
Let $f:M^3 \to M^3$ be a $C^2$-diffeomorphism and let $\Lambda$ be a hyperbolic attractor as above. Suppose that $\Lambda$ also verifies the following properties:
\begin{enumerate}
\item[(a)] $\Lambda$ is usu-accessible;
\item[(b)] there exists $\varepsilon>0$ such that for any $x\in \Lambda$ and $y\in \cW^s_{\varepsilon}(x) \cap \Lambda$ it holds that $\alpha^s(x,y) \neq 0$.
\end{enumerate}
Then the strong unstable lamination is minimal in $\Lambda$ and every $u$-Gibbs measure is SRB.
\end{theorem}

We say that a set $K\subset \Lambda$ is $\mathcal{W}^u$-minimal if any $x\in K$ verifies that $W^u(x) \subset K$ and $\overline{W^u(x)} = K$. 
In \cite{RHUres}, Rodriguez Hertz and Ures study the usu-property for partially hyperbolic diffeomorphisms, and they prove the following theorem.
\begin{theorem}[Theorem 1.1, \cite{RHUres}]
\label{thm.usuminimality}
If $g$ is an usu-accessible partially hyperbolic diffeomorphism,  then $\mathcal{W}^u$ has a unique minimal set. 
\end{theorem} 
Even though, the authors prove this theorem for partially hyperbolic diffeomorphisms, the same proof holds in our setting (see \cite{RHUres}).  In particular, the following statement is true.
\begin{lemma}
\label{lem.usuminimal}
Let $f:M^3 \to M^3$ be a $C^1$-diffeomorphisms and let $\Lambda$ be a hyperbolic attractor having a dominated splitting $T_{\Lambda}M = E^s \oplus E^c \oplus E^u$. Suppose that $\Lambda$ is usu-accessible. Then strong unstable lamination $\mathcal{W}^u$ has a unique minimal set in $\Lambda$. 
\end{lemma}

\begin{proof}[Proof of Theorem \ref{thm.attractorusu}]
By Lemma \ref{lem.usuminimal}, there exists a unique set $K \subset \Lambda$ which is a minimal set of the lamination $\mathcal{W}^u$.  Since the image of a $\mathcal{W}^u$-minimal set is $\mathcal{W}^u$-minimal, by uniqueness of the minimal set  $f(K) = K$.  The invariance of $K$ and the fact that $K$ is $u$-saturated allow us to find $u$-Gibbs measures that are supported on $K$. Since $K$ is $\mathcal{W}^u$-minimal, we have that any $u$-Gibbs measure $\mu$ supported on $K$ verifies $\mathrm{supp}(\mu) = K$. 

Let $\mu$ be an ergodic $u$-Gibbs measure supported on $K$.  Condition $(b)$ in the hypothesis of Theorem \ref{thm.attractorusu} implies that $\mu(\mathbf{B}) = 0$. By Theorem \ref{thm. mainthmforattractors}, we obtain that $\mu$ is SRB. 

We claim that $\Lambda$ is transitive.  Otherwise we could decompose $\Lambda$ into at least two different invariant parts, each of which would support a minimal set for $\mathcal{W}^u$ and this would contradict the uniqueness of the minimal set. 

Since $\Lambda$ is transitive, there exists a unique SRB measure and this measure has full support. In particular, we conclude that $\mu$ is this unique measure and $\mathrm{supp}(\mu) = \Lambda$. Since $\mu$ was supported in $K$, we conclude that $K = \Lambda$ and the strong unstable lamination is minimal in $\Lambda$. 

Now, if $\nu$ is any other $u$-Gibbs measure supported in $\Lambda$, the since the strong unstable lamination is minimal, we have that $\mathrm{supp}(\nu) = \Lambda$. By Theorem \ref{thm.fullsupportmainthmattractors} and since $\Lambda$ is accessible, $\nu$ is SRB. In particular, there exists only one $u$-Gibbs measure which is the SRB measure. \qedhere


\end{proof}

Things missing:
\begin{itemize}
\item Write the points from section $3$ to adapt the proof of Theorem \ref{thm.fullsupportmainthmattractors};
\item Describe an example that verifies the hypothesis of Theorem \ref{thm.usuminimality}
\end{itemize}

==> Sec9_final.tex <==
fasd

==> final.tex <==
fasd
